On the Change in Archivability of Websites Over Time

As web technologies evolve, web archivists work to keep up so that our digital history is preserved. Recent advances in web technologies have introduced client-side executed scripts that load data without a referential identifier or that require user interaction (e.g., content loading when the page has scrolled). These advances have made automating methods for capturing web pages more difficult. Because of the evolving schemes of publishing web pages along with the progressive capability of web preservation tools, the archivability of pages on the web has varied over time. In this paper we show that the archivability of a web page can be deduced from the type of page being archived, which aligns with that page's accessibility in respect to dynamic content. We show concrete examples of when these technologies were introduced by referencing mementos of pages that have persisted through a long evolution of available technologies. Identifying these reasons for the inability of these web pages to be archived in the past in respect to accessibility serves as a guide for ensuring that content that has longevity is published using good practice methods that make it available for preservation.

==> justin <==
[General]
cookies="@Variant(\0\0\0\x7f\0\0\0\x16QList<QNetworkCookie>\0\0\0\0\x1\0\0\0\x3\0\0\0\x81wayback_server=37; expires=Thu, 14-Feb-2013 19:41:06 GMT; domain=.archive.org; path=/memento/20010506102951/http%3A//www.cnn.com/\0\0\0`EditionPopUp=seen(sh:0&id:0); expires=Tue, 22-Jan-2013 19:41:12 GMT; domain=.archive.org; path=/\0\0\0jCNNid=G3c0aaf82-50f5b0d3-001e72b4-03030b02; expires=Tue, 22-Jan-2013 19:41:07 GMT; domain=.cnn.com; path=/)"

